Prospects for the observation of continuous gravitational waves from spinning neutron stars lensed by the galactic supermassive black hole

We study the prospects of detecting continuous gravitational waves (CGWs) from spinning neutron stars (NSs), gravitationally lensed by the galactic supermassive black hole. Assuming various astrophysically motivated spatial distributions of galactic NSs, we find that CGW signals from a few ($\sim 0-6$) neutron stars should be strongly lensed. Lensing will produce two copies of the signal (with time delays of seconds to minutes) that will interfere with each other. The relative motion of the NS with respect to the lensing optical axis will change the interference pattern, which will help us to identify a lensed signal. Accounting for the magnifications and time delays of the lensed signals, we investigate their detectability by ground-based detectors. Modelling the spin distribution of NSs based on that of known pulsars and assuming an ellipticity of $\epsilon = 10^{-7}$, lensed CGWs are unlikely to be detectable by LIGO and Virgo in realistic searches involving $\mathcal{O}(10^{12})$ templates. However, third generation detectors have a $\sim 2-51\%$ probability of detecting at least one lensed CGW signal. For an ellipticity of $\epsilon = 10^{-8}$, the detection probability reduces to $\sim 0-18 \, \% $. Though rare, such an observation will enable interesting probes of the supermassive black hole and its environment.

==> arXiv Resubmission/macros.tex <==
%%% General purpose macros
\newcommand{\ffrac}[2]{\ensuremath{\frac{\displaystyle #1}
                                        {\displaystyle #2}}}

\def\frmrtHz{\frac{\rm m}{\rtHz}}
\def\Msol{\ensuremath{\mathit{M_\odot}}}
\def\Msun{\Msol}
\def\Mcc{\Msol \ensuremath{\mathit{c}^2}}
\newcommand{\Mc}{\ensuremath{\mathcal{M}_c}}
\newcommand{\chieff}{\ensuremath{\chi_\mathrm{eff}}}

%%% New symbols and commands
\newcommand{\Ylm}{\ensuremath{Y_{\ell m}^{-2}(\iota, \varphi_{o})}}
\newcommand{\blambda}{\pmb{\lambda}}


%%% Various constants/measurements/units
\newcommand{\numevents}{56}
\newcommand{\sqdeg}{\ensuremath{\text{deg}^2}}

